Data Poisoning Attacks to Locally Differentially Private Frequent Itemset Mining Protocols

Local differential privacy (LDP) provides a way for an untrusted data collector to aggregate users' data without violating their privacy. Various privacy-preserving data analysis tasks have been studied under the protection of LDP, such as frequency estimation, frequent itemset mining, and machine learning. Despite its privacy-preserving properties, recent research has demonstrated the vulnerability of certain LDP protocols to data poisoning attacks. However, existing data poisoning attacks are focused on basic statistics under LDP, such as frequency estimation and mean/variance estimation. As an important data analysis task, the security of LDP frequent itemset mining has yet to be thoroughly examined. In this paper, we aim to address this issue by presenting novel and practical data poisoning attacks against LDP frequent itemset mining protocols. By introducing a unified attack framework with composable attack operations, our data poisoning attack can successfully manipulate the state-of-the-art LDP frequent itemset mining protocols and has the potential to be adapted to other protocols with similar structures. We conduct extensive experiments on three datasets to compare the proposed attack with four baseline attacks. The results demonstrate the severity of the threat and the effectiveness of the proposed attack.

==> sec_threat.tex <==
\section{Threat Model}
\subsection{Assumptions}
For the attacker's capability, we follow the assumption made by previous work that the attacker can inject/corrupt users and let them report any arbitrary values  that obey the formats of LDP protocols to the aggregator~\cite{DBLP:conf/uss/CaoJG21, DBLP:conf/sp/CheuSU21} . The corrupted users can craft the original values, encoded values, and the perturbed values. We assume that the attacker can inject/corrupt at most $m \leq n$  users. If we assume that the attacker will inject/corrupt as many users as possible, then we have that the number of honest user is $n - m$. Denoted by the set of benign users by $U^b$, and the set of corrupted users by $U^c$.

We also assume that the attacker knows the pre-defined parameters of the LDP protocols. Because the aggregator has no idea which user is corrupted or honest, it will share the implementation/setting to every user for running the LDP protocols. However, the attacker has no prior knowledge about the parameters that are adaptively determined by the protocols. In addition, we assume that the attacker knows the original values of the corrupted users.
%the frequencies of the targeted items/itemsets and the threshold for the top-$k$ item.

Suppose that there is a set of target items $T = \{t_1, t_2, \ldots, t_{|T|}\}$. To get the items in $T$ into the result of frequent item mining, the attacker carefully selects the responses to the aggregator in the interactive process of the LDP protocol. Denoted by the set of responses of all user $\mathcal{R}$, the set of responses of all benign users $\mathcal{R}^b$, and the set of responses of all corrupted users $\mathcal{R}^c$. For each user $j$, the response $R_j \in \mathcal{R}$ is a sequence of perturbed values $y_{j,1}, y_{j,2}, \ldots$ generated by the LDP protocol.

More specifically, we consider three different types of attackers that have different levels of knowledge about the information regarding frequent itemset mining process:
\begin{itemize}
    \item Omniscient Attacker: The omniscient attack (OA) assumes that the attacker knows the true frequencies of all items/itemsets. Though the assumption is somewhat strong, there are some scenarios where it is applicable. For example, there are two aggregators that are competitors. One of them has completed the data aggregation and wants to prevent the other from mining the (genuine) frequent items.
    \item Surrogate  Attacker : 
    \item Imitation Attacker:
\end{itemize}


\subsection{Attack Goals} 
Suppose that an attacker tries to manipulate the top-$k$ frequent item(set) mining results by make some target items into the results.

The attacker tries to measure the probability
\begin{equation}\label{eq:propattack}
  \Pr[\tilde{f}^*(t) > \tilde{f}^*_{k+1}].
\end{equation}
where $\tilde{f}^*(t)$ is the frequency of item $t$ after the attack, and $\tilde{f}^*_{k+1}$ is the $(k+1)$-th high frequency among all the items.

We assume that the attacker usually has three different goals:
\begin{itemize}
 \item The first goal is to decrease the accuracy of the resulting model, which is equivalent to the first goal by setting all items except the true top-$k$ items as the target items. Yet, we put it up as another goal, because in usual case, this is an oriented purpose of attackers. Formally, this objective can be formulated as
      \begin{equation}\label{eq:goal3}
        \text{minimize}\quad \sum_{t\in \mathcal{I}_k}\mathbb{1}(\tilde{f}^*(t) > \tilde{f}^*_{k+1})
      \end{equation}
    where $\mathcal{I}_k$ is the set of true top-$k$ items before the attack. We treat the attacks with this goal as \textit{Untargeted Attacks} (UTA). 
    
  \item The second goal is to get as many items in $T$ as possible into the top-$k$ frequent items. Formally, this objective can be formulated as
      \begin{equation}\label{eq:goal1}
        \text{maximize}\quad \sum_{t\in T}\mathbb{1}(\tilde{f}^*(t) > \tilde{f}^*_{k+1}),
      \end{equation}
      where $\mathbb{1}(\mathsf{cond})$ is an indicator function that returns 1 if $\mathsf{cond}$ is true; otherwise 0. We name the attacks with this goal as \textit{Targeted Attack type-\rom{1}} (TA1).
  \item The third goal is to get some items in $T$ to achieve as top ranking as possible. Formally, this objective can be formulated as
      \begin{equation}\label{eq:goal2}
        \max_{t\in T} \arg\max_{k^t}  (\tilde{f}^*(t) > \tilde{f}^*_{k^t}).
      \end{equation}
      This type of attacks is called as \textit{Targeted Attack type-\rom{2}} (TA2).
   
\end{itemize}
